Detecting Diffusion-Generated Time Series Under Generator Shift

The boundary between real and diffusion-generated time series is becoming increasingly difficult to draw, yet detection in this domain remains underexplored, especially when the generator is unknown. We compare white-box detection, which requires access to the generator, against black-box detection, which operates on the raw signal alone. The white-box approach, a reconstruction-based detector adapted from the image domain, works well in in-distribution but breaks down under generator shift: reconstruction-based detection in images succeeds because large generic generators provide a near-universal reconstruction prior, and no analogous generator exists for time series. In contrast, a simple off-the-shelf classifier used as a black-box detector performs remarkably well, achieving an average F1 of 79.2, a 22.1% relative improvement over the white-box approach, and a TPR@1%FPR of 57.2. Diffusion-generated time series detection is therefore not a direct transfer of the image domain problem. This work provides the first systematic exploration of white-box and black-box detection for diffusion-generated time series. We close by identifying several open and promising directions.

==> src/tables/dataset_128.tex <==
\begin{table}[ht!]
% \setlength{\tabcolsep}{4pt}
\caption{Detectability across ten datasets for \textit{128-length} sequences. All metrics are higher the better, with TPR measured at a 1\% FPR. Values in \textcolor{gray}{gray} are ID, while values in black are OOD. The best average OOD scores are highlighted in \colorbox{green!15}{green}.}
\label{tab:dataset_128}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llccccccccccccccc}

\toprule

& & \multicolumn{5}{c}{Electricity} & \multicolumn{5}{c}{Energy} & \multicolumn{5}{c}{ETTh1} \\

\cmidrule(r){3-7}
\cmidrule(rl){8-12}
\cmidrule(l){13-17}

Generator & Method & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ \\

\midrule

\multirow{2}{*}{SSSD} & DIRE & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{98.0} & \textcolor{gray}{98.0} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{99.2} & \textcolor{gray}{99.7} & \textcolor{gray}{99.7} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{99.9} \\
& Disjoint-CNN & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{98.8} & \textcolor{gray}{98.9} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
\cmidrule{1-17}

\multirow{2}{*}{TSDiff} & DIRE & 66.6 & 50.0 & 49.8 & 49.6 & 0.00 & 65.2 & 48.7 & 48.1 & 46.2 & 0.00 & 67.8 & 52.8 & 54.1 & 57.5 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 100. & 100. & 100. & 66.7 & 50.0 & 75.8 & 80.4 & 4.88 & 65.6 & 48.9 & 60.9 & 51.1 & 7.03 \\
\cmidrule{1-17}

\multirow{2}{*}{Diffusion-TS} & DIRE & 66.6 & 50.0 & 49.8 & 49.6 & 0.00 & 64.9 & 48.1 & 47.4 & 44.7 & 0.00 & 66.5 & 49.8 & 49.6 & 49.2 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 30.9 & 0.76 & 0.00 & 66.7 & 50.0 & 58.5 & 60.3 & 2.34 & 65.6 & 48.9 & 37.8 & 27.2 & 0.00 \\
\cmidrule{1-17}

\multirow{2}{*}{WaveStitch} & DIRE & 67.1 & 51.0 & 56.3 & 61.1 & 0.00 & 65.2 & 48.6 & 48.7 & 47.5 & 0.00 & 68.5 & 54.1 & 59.8 & 66.2 & 0.00 \\
& Disjoint-CNN & 99.6 & 99.6 & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 65.6 & 48.9 & 70.7 & 68.5 & 0.48 \\
\cmidrule{1-17}

\multirow{2}{*}{Avg. OOD} & DIRE & 66.8 & 50.3 & 52.0 & 53.4 & 0.00 & 65.1 & 48.5 & 48.1 & 46.2 & 0.00 & \cellcolor{green!15}{67.6} & \cellcolor{green!15}{52.2} & 54.5 & \cellcolor{green!15}{57.6} & 0.00 \\
& Disjoint-CNN & \cellcolor{green!15}{77.7} & \cellcolor{green!15}{66.5} & \cellcolor{green!15}{77.0} & \cellcolor{green!15}{66.9} & \cellcolor{green!15}{66.7} & \cellcolor{green!15}{77.8} & \cellcolor{green!15}{66.7} & \cellcolor{green!15}{78.1} & \cellcolor{green!15}{80.2} & \cellcolor{green!15}{35.7} & 65.6 & 48.9 & \cellcolor{green!15}{56.5} & 48.9 & \cellcolor{green!15}{2.50} \\

\bottomrule

\toprule

& & \multicolumn{5}{c}{ETTm1} & \multicolumn{5}{c}{Exchange Rate} & \multicolumn{5}{c}{fMRI} \\

\cmidrule(r){3-7}
\cmidrule(rl){8-12}
\cmidrule(l){13-17}

Generator & Method & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ \\

\midrule

\multirow{2}{*}{SSSD} & DIRE & \textcolor{gray}{99.5} & \textcolor{gray}{99.5} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{99.9} & \textcolor{gray}{81.7} & \textcolor{gray}{84.5} & \textcolor{gray}{99.6} & \textcolor{gray}{99.7} & \textcolor{gray}{98.3} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
& Disjoint-CNN & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
\cmidrule{1-17}

\multirow{2}{*}{TSDiff} & DIRE & 66.3 & 49.6 & 47.1 & 44.3 & 0.00 & 52.6 & 37.4 & 33.3 & 15.6 & 0.00 & 66.7 & 50.0 & 85.4 & 90.4 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 53.9 & 58.1 & 1.93 & 67.0 & 50.8 & 100. & 100. & 98.7 & 66.7 & 50.0 & 99.9 & 99.9 & 97.4 \\
\cmidrule{1-17}

\multirow{2}{*}{Diffusion-TS} & DIRE & 66.3 & 49.6 & 47.4 & 45.0 & 0.00 & 52.0 & 35.9 & 32.2 & 10.8 & 0.00 & 66.7 & 50.0 & 48.9 & 47.9 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 46.5 & 44.2 & 0.03 & 67.6 & 52.0 & 98.3 & 97.7 & 92.4 & 66.7 & 50.0 & 44.3 & 40.7 & 2.12 \\
\cmidrule{1-17}

\multirow{2}{*}{WaveStitch} & DIRE & 66.2 & 49.5 & 60.3 & 65.2 & 0.00 & 54.0 & 41.0 & 34.5 & 19.9 & 0.00 & 66.7 & 50.0 & 56.0 & 60.5 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 93.8 & 95.7 & 17.0 & 66.7 & 50.0 & 70.8 & 66.1 & 14.0 & 94.5 & 94.2 & 100. & 100. & 100. \\
\cmidrule{1-17}

\multirow{2}{*}{Avg. OOD} & DIRE & 66.3 & 49.6 & 51.6 & 51.5 & 0.00 & 52.9 & 38.1 & 33.3 & 15.4 & 0.00 & 66.7 & 50.0 & 63.4 & 66.2 & 0.00 \\
& Disjoint-CNN & \cellcolor{green!15}{66.7} & \cellcolor{green!15}{50.0} & \cellcolor{green!15}{64.7} & \cellcolor{green!15}{66.0} & \cellcolor{green!15}{6.31} & \cellcolor{green!15}{67.1} & \cellcolor{green!15}{50.9} & \cellcolor{green!15}{89.7} & \cellcolor{green!15}{87.9} & \cellcolor{green!15}{68.4} & \cellcolor{green!15}{75.9} & \cellcolor{green!15}{64.7} & \cellcolor{green!15}{81.4} & \cellcolor{green!15}{80.2} & \cellcolor{green!15}{66.5} \\

\bottomrule

\toprule

& & \multicolumn{5}{c}{Illness} & \multicolumn{5}{c}{Stock} & \multicolumn{5}{c}{Traffic} \\

\cmidrule(r){3-7}
\cmidrule(rl){8-12}
\cmidrule(l){13-17}

Generator & Method & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ \\

\midrule

\multirow{2}{*}{SSSD} & DIRE & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{1.46} & \textcolor{gray}{50.0} & \textcolor{gray}{52.2} & \textcolor{gray}{55.5} & \textcolor{gray}{1.34} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
& Disjoint-CNN & \textcolor{gray}{48.5} & \textcolor{gray}{66.0} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
\cmidrule{1-17}

\multirow{2}{*}{TSDiff} & DIRE & 66.7 & 50.0 & 51.2 & 56.7 & 0.00 & 0.93 & 21.0 & 31.6 & 6.67 & 0.00 & 66.7 & 50.0 & 50.0 & 50.0 & 0.00 \\
& Disjoint-CNN & 38.1 & 47.9 & 62.3 & 64.0 & 12.4 & 66.7 & 50.0 & 78.0 & 62.5 & 55.2 & 66.7 & 50.0 & 100. & 100. & 100. \\
\cmidrule{1-17}

\multirow{2}{*}{Diffusion-TS} & DIRE & 66.7 & 50.0 & 34.9 & 18.5 & 0.00 & 0.75 & 1.60 & 30.7 & 0.11 & 0.00 & 66.7 & 50.1 & 50.0 & 50.1 & 0.00 \\
& Disjoint-CNN & 28.0 & 17.8 & 37.1 & 13.6 & 3.86 & 66.7 & 50.0 & 30.8 & 2.32 & 0.00 & 66.7 & 50.1 & 40.3 & 37.5 & 0.00 \\
\cmidrule{1-17}

\multirow{2}{*}{WaveStitch} & DIRE & 66.7 & 50.0 & 81.3 & 79.8 & 20.1 & 1.34 & 45.4 & 41.2 & 41.3 & 0.00 & 66.7 & 50.0 & 50.1 & 50.1 & 0.00 \\
& Disjoint-CNN & 48.5 & 66.0 & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. \\
\cmidrule{1-17}

\multirow{2}{*}{Avg. OOD} & DIRE & \cellcolor{green!15}{66.7} & \cellcolor{green!15}{50.0} & 55.8 & 51.7 & 6.69 & 1.01 & 22.6 & 34.5 & 16.0 & 0.00 & 66.7 & 50.0 & 50.0 & 50.1 & 0.00 \\
& Disjoint-CNN & 38.2 & 43.9 & \cellcolor{green!15}{66.5} & \cellcolor{green!15}{59.2} & \cellcolor{green!15}{38.7} & \cellcolor{green!15}{77.8} & \cellcolor{green!15}{66.7} & \cellcolor{green!15}{69.6} & \cellcolor{green!15}{55.0} & \cellcolor{green!15}{51.7} & \cellcolor{green!15}{77.8} & \cellcolor{green!15}{66.7} & \cellcolor{green!15}{80.1} & \cellcolor{green!15}{79.2} & \cellcolor{green!15}{66.7} \\

\bottomrule

\toprule

& & \multicolumn{5}{c}{Weather} \\

\cmidrule{3-17}

Generator & Method & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ \\

\midrule

\multirow{2}{*}{SSSD} & DIRE & \textcolor{gray}{99.7} & \textcolor{gray}{99.7} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{99.9} \\
& Disjoint-CNN & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
\cmidrule{1-17}

\multirow{2}{*}{TSDiff} & DIRE & 66.4 & 49.7 & 49.7 & 49.4 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 88.4 & 83.8 & 49.7 \\
\cmidrule{1-17}

\multirow{2}{*}{Diffusion-TS} & DIRE & 66.4 & 49.7 & 49.7 & 49.5 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 42.8 & 37.2 & 0.99 \\
\cmidrule{1-17}

\multirow{2}{*}{WaveStitch} & DIRE & 73.7 & 64.5 & 64.5 & 72.3 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 100. & 100. & 99.9 \\
\cmidrule{1-17}

\multirow{2}{*}{Avg. OOD} & DIRE & \cellcolor{green!15}{68.8} & \cellcolor{green!15}{54.6} & 54.6 & 57.1 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & \cellcolor{green!15}{77.1} & \cellcolor{green!15}{73.7} & \cellcolor{green!15}{50.2} \\

\bottomrule
\end{tabular}
}
\end{table}

==> src/tables/dataset_32.tex <==
\begin{table}[ht!]
% \setlength{\tabcolsep}{4pt}
\caption{Detectability across ten datasets for \textit{32-length} sequences. All metrics are higher the better, with TPR measured at a 1\% FPR. Values in \textcolor{gray}{gray} are ID, while values in black are OOD. The best average OOD scores are highlighted in \colorbox{green!15}{green}.}
\label{tab:dataset_32}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llccccccccccccccc}

\toprule

& & \multicolumn{5}{c}{Electricity} & \multicolumn{5}{c}{Energy} & \multicolumn{5}{c}{ETTh1} \\

\cmidrule(r){3-7}
\cmidrule(rl){8-12}
\cmidrule(l){13-17}

Generator & Method & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ \\

\midrule

\multirow{2}{*}{SSSD} & DIRE & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{74.9} & \textcolor{gray}{79.7} & \textcolor{gray}{95.6} & \textcolor{gray}{94.8} & \textcolor{gray}{57.6} \\
& Disjoint-CNN & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{99.9} & \textcolor{gray}{99.9} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{99.9} \\
\cmidrule{1-17}

\multirow{2}{*}{TSDiff} & DIRE & 66.7 & 50.0 & 50.0 & 50.0 & 0.00 & 66.7 & 50.0 & 50.0 & 50.0 & 0.00 & 47.1 & 32.0 & 35.4 & 20.1 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 99.6 & 99.7 & 98.2 & 66.7 & 50.0 & 63.0 & 62.3 & 4.71 & 94.2 & 93.9 & 99.9 & 99.9 & 99.8 \\
\cmidrule{1-17}

\multirow{2}{*}{Diffusion-TS} & DIRE & 92.4 & 91.8 & 96.3 & 98.1 & 0.00 & 66.7 & 50.0 & 50.2 & 50.3 & 0.00 & 55.8 & 52.0 & 51.8 & 54.6 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 31.0 & 3.50 & 0.00 & 66.7 & 50.0 & 40.6 & 34.6 & 0.52 & 77.5 & 71.1 & 95.5 & 95.6 & 55.7 \\
\cmidrule{1-17}

\multirow{2}{*}{WaveStitch} & DIRE & 66.7 & 50.0 & 50.0 & 50.0 & 0.00 & 83.1 & 79.7 & 90.0 & 94.5 & 0.00 & 49.2 & 37.4 & 54.5 & 44.3 & 0.00 \\
& Disjoint-CNN & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 99.5 & 99.5 & 100. & 100. & 99.9 \\
\cmidrule{1-17}

\multirow{2}{*}{Avg. OOD} & DIRE & 75.2 & 63.9 & 65.4 & 66.0 & 0.00 & 72.1 & 59.9 & 63.4 & 64.9 & 0.00 & 50.7 & 40.5 & 47.2 & 39.7 & 0.00 \\
& Disjoint-CNN & \cellcolor{green!15}{77.8} & \cellcolor{green!15}{66.7} & \cellcolor{green!15}{76.9} & \cellcolor{green!15}{67.7} & \cellcolor{green!15}{66.1} & \cellcolor{green!15}{77.8} & \cellcolor{green!15}{66.7} & \cellcolor{green!15}{67.9} & \cellcolor{green!15}{65.7} & \cellcolor{green!15}{35.1} & \cellcolor{green!15}{90.4} & \cellcolor{green!15}{88.1} & \cellcolor{green!15}{98.5} & \cellcolor{green!15}{98.5} & \cellcolor{green!15}{85.1} \\

\bottomrule

\toprule

& & \multicolumn{5}{c}{ETTm1} & \multicolumn{5}{c}{Exchange Rate} & \multicolumn{5}{c}{fMRI} \\

\cmidrule(r){3-7}
\cmidrule(rl){8-12}
\cmidrule(l){13-17}

Generator & Method & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ \\

\midrule

\multirow{2}{*}{SSSD} & DIRE & \textcolor{gray}{98.8} & \textcolor{gray}{98.9} & \textcolor{gray}{99.2} & \textcolor{gray}{98.6} & \textcolor{gray}{98.3} & \textcolor{gray}{68.8} & \textcolor{gray}{76.2} & \textcolor{gray}{98.8} & \textcolor{gray}{99.0} & \textcolor{gray}{74.1} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
& Disjoint-CNN & \textcolor{gray}{98.1} & \textcolor{gray}{98.1} & \textcolor{gray}{99.9} & \textcolor{gray}{99.8} & \textcolor{gray}{98.2} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
\cmidrule{1-17}

\multirow{2}{*}{TSDiff} & DIRE & 72.3 & 62.5 & 76.3 & 83.4 & 0.00 & 41.6 & 26.3 & 30.9 & 3.21 & 0.00 & 66.7 & 50.0 & 79.3 & 87.0 & 0.00 \\
& Disjoint-CNN & 92.6 & 92.3 & 99.0 & 98.7 & 91.9 & 74.5 & 65.7 & 97.5 & 97.8 & 54.4 & 100. & 100. & 100. & 100. & 100. \\
\cmidrule{1-17}

\multirow{2}{*}{Diffusion-TS} & DIRE & 67.1 & 51.9 & 56.2 & 60.6 & 0.00 & 46.2 & 38.7 & 37.5 & 29.6 & 0.00 & 66.7 & 50.0 & 50.0 & 50.0 & 0.00 \\
& Disjoint-CNN & 65.0 & 48.2 & 70.3 & 71.5 & 0.00 & 77.2 & 70.5 & 89.4 & 90.3 & 35.5 & 66.7 & 50.0 & 62.2 & 62.8 & 3.43 \\
\cmidrule{1-17}

\multirow{2}{*}{WaveStitch} & DIRE & 95.4 & 95.3 & 97.7 & 97.7 & 0.00 & 62.4 & 68.4 & 70.3 & 80.4 & 0.00 & 100. & 100. & 100. & 100. & 100. \\
& Disjoint-CNN & 97.1 & 97.1 & 99.6 & 99.6 & 95.7 & 99.9 & 99.9 & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. \\
\cmidrule{1-17}

\multirow{2}{*}{Avg. OOD} & DIRE & 78.2 & 69.9 & 76.8 & 80.6 & 0.00 & 50.1 & 44.5 & 46.2 & 37.8 & 0.00 & 77.8 & 66.7 & 76.4 & 79.0 & 33.3 \\
& Disjoint-CNN & \cellcolor{green!15}{84.9} & \cellcolor{green!15}{79.2} & \cellcolor{green!15}{89.6} & \cellcolor{green!15}{89.9} & \cellcolor{green!15}{62.5} & \cellcolor{green!15}{83.9} & \cellcolor{green!15}{78.7} & \cellcolor{green!15}{95.6} & \cellcolor{green!15}{96.0} & \cellcolor{green!15}{63.3} & \cellcolor{green!15}{88.9} & \cellcolor{green!15}{83.3} & \cellcolor{green!15}{87.4} & \cellcolor{green!15}{87.6} & \cellcolor{green!15}{67.8} \\

\bottomrule

\toprule

& & \multicolumn{5}{c}{Illness} & \multicolumn{5}{c}{Stock} & \multicolumn{5}{c}{Traffic} \\

\cmidrule(r){3-7}
\cmidrule(rl){8-12}
\cmidrule(l){13-17}

Generator & Method & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ \\

\midrule

\multirow{2}{*}{SSSD} & DIRE & \textcolor{gray}{99.4} & \textcolor{gray}{99.4} & \textcolor{gray}{99.4} & \textcolor{gray}{99.7} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
& Disjoint-CNN & \textcolor{gray}{99.0} & \textcolor{gray}{99.0} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
\cmidrule{1-17}

\multirow{2}{*}{TSDiff} & DIRE & 66.7 & 50.1 & 50.1 & 50.1 & 0.00 & 66.7 & 50.0 & 50.0 & 50.0 & 0.00 & 66.7 & 50.0 & 50.0 & 50.0 & 0.00 \\
& Disjoint-CNN & 96.7 & 96.6 & 100. & 100. & 99.4 & 100. & 100. & 100. & 100. & 100. & 66.7 & 50.0 & 93.4 & 95.8 & 18.2 \\
\cmidrule{1-17}

\multirow{2}{*}{Diffusion-TS} & DIRE & 67.7 & 52.3 & 52.2 & 54.2 & 0.00 & 66.9 & 50.5 & 52.1 & 54.0 & 0.00 & 91.5 & 90.7 & 89.2 & 94.0 & 0.00 \\
& Disjoint-CNN & 92.9 & 92.4 & 100. & 100. & 99.2 & 71.3 & 59.8 & 39.9 & 38.3 & 0.00 & 66.7 & 50.1 & 36.8 & 27.6 & 0.30 \\
\cmidrule{1-17}

\multirow{2}{*}{WaveStitch} & DIRE & 66.9 & 50.4 & 68.7 & 77.2 & 0.00 & 95.3 & 95.1 & 96.0 & 97.9 & 0.00 & 66.7 & 50.0 & 50.0 & 50.0 & 0.00 \\
& Disjoint-CNN & 88.4 & 86.9 & 99.8 & 99.8 & 96.3 & 99.6 & 99.6 & 99.6 & 99.8 & 100. & 100. & 100. & 100. & 100. & 100. \\
\cmidrule{1-17}

\multirow{2}{*}{Avg. OOD} & DIRE & 67.1 & 50.9 & 57.0 & 60.5 & 0.00 & 76.3 & 65.2 & 66.0 & 67.3 & 0.00 & 74.9 & 63.6 & 63.1 & 64.7 & 0.00 \\
& Disjoint-CNN & \cellcolor{green!15}{92.7} & \cellcolor{green!15}{92.0} & \cellcolor{green!15}{99.9} & \cellcolor{green!15}{99.9} & \cellcolor{green!15}{98.3} & \cellcolor{green!15}{90.3} & \cellcolor{green!15}{86.5} & \cellcolor{green!15}{79.8} & \cellcolor{green!15}{79.4} & \cellcolor{green!15}{66.7} & \cellcolor{green!15}{77.8} & \cellcolor{green!15}{66.7} & \cellcolor{green!15}{76.7} & \cellcolor{green!15}{74.5} & \cellcolor{green!15}{39.5} \\

\bottomrule

\toprule

& & \multicolumn{5}{c}{Weather} \\

\cmidrule{3-17}

Generator & Method & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ \\

\midrule

\multirow{2}{*}{SSSD} & DIRE & \textcolor{gray}{99.9} & \textcolor{gray}{99.9} & \textcolor{gray}{100.} & \textcolor{gray}{99.9} & \textcolor{gray}{100.} \\
& Disjoint-CNN & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
\cmidrule{1-17}

\multirow{2}{*}{TSDiff} & DIRE & 66.6 & 49.9 & 47.7 & 45.3 & 0.00 \\
& Disjoint-CNN & 83.1 & 79.7 & 99.9 & 99.9 & 98.2 \\
\cmidrule{1-17}

\multirow{2}{*}{Diffusion-TS} & DIRE & 66.7 & 50.1 & 51.8 & 53.3 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 52.9 & 54.0 & 1.06 \\
\cmidrule{1-17}

\multirow{2}{*}{WaveStitch} & DIRE & 78.4 & 72.4 & 97.9 & 98.7 & 0.00 \\
& Disjoint-CNN & 100. & 100. & 100. & 100. & 100. \\
\cmidrule{1-17}

\multirow{2}{*}{Avg. OOD} & DIRE & 70.5 & 57.5 & 65.8 & 65.8 & 0.00 \\
& Disjoint-CNN & \cellcolor{green!15}{83.3} & \cellcolor{green!15}{76.6} & \cellcolor{green!15}{84.3} & \cellcolor{green!15}{84.6} & \cellcolor{green!15}{66.4} \\

\bottomrule
\end{tabular}
}
\end{table}

==> src/tables/dataset_64.tex <==
\begin{table}[ht!]
% \setlength{\tabcolsep}{4pt}
\caption{Detectability across ten datasets for \textit{64-length} sequences. All metrics are higher the better, with TPR measured at a 1\% FPR. Values in \textcolor{gray}{gray} are ID, while values in black are OOD. The best average OOD scores are highlighted in \colorbox{green!15}{green}.}
\label{tab:dataset_64}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llccccccccccccccc}

\toprule

& & \multicolumn{5}{c}{Electricity} & \multicolumn{5}{c}{Energy} & \multicolumn{5}{c}{ETTh1} \\

\cmidrule(r){3-7}
\cmidrule(rl){8-12}
\cmidrule(l){13-17}

Generator & Method & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ \\

\midrule

\multirow{2}{*}{SSSD} & DIRE & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{79.7} & \textcolor{gray}{83.0} & \textcolor{gray}{97.4} & \textcolor{gray}{97.4} & \textcolor{gray}{71.8} \\
& Disjoint-CNN & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
\cmidrule{1-17}

\multirow{2}{*}{TSDiff} & DIRE & 66.7 & 50.0 & 50.0 & 50.0 & 0.00 & 66.7 & 50.0 & 50.0 & 50.0 & 0.00 & 63.5 & 61.7 & 58.0 & 66.0 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 100. & 100. & 100. & 66.7 & 50.0 & 99.5 & 99.4 & 92.1 & 90.4 & 89.4 & 99.9 & 99.9 & 98.0 \\
\cmidrule{1-17}

\multirow{2}{*}{Diffusion-TS} & DIRE & 85.2 & 82.6 & 95.0 & 97.4 & 0.00 & 66.8 & 50.4 & 50.6 & 51.2 & 0.00 & 62.4 & 59.8 & 57.3 & 63.6 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 31.1 & 1.83 & 0.00 & 66.7 & 50.0 & 46.8 & 43.4 & 1.34 & 73.3 & 63.5 & 95.5 & 96.5 & 37.4 \\
\cmidrule{1-17}

\multirow{2}{*}{WaveStitch} & DIRE & 66.7 & 50.0 & 50.0 & 50.0 & 0.00 & 85.0 & 82.3 & 88.8 & 93.7 & 0.00 & 54.2 & 43.6 & 52.9 & 49.7 & 0.00 \\
& Disjoint-CNN & 100. & 100. & 100. & 100. & 100. & 96.0 & 95.8 & 99.8 & 99.9 & 99.9 & 99.5 & 99.5 & 100. & 100. & 100. \\
\cmidrule{1-17}

\multirow{2}{*}{Avg. OOD} & DIRE & 72.8 & 60.9 & 65.0 & 65.8 & 0.00 & 72.8 & 60.9 & 63.1 & 64.9 & 0.00 & 60.1 & 55.0 & 56.1 & 59.8 & 0.00 \\
& Disjoint-CNN & \cellcolor{green!15}{77.8} & \cellcolor{green!15}{66.7} & \cellcolor{green!15}{77.0} & \cellcolor{green!15}{67.3} & \cellcolor{green!15}{66.7} & \cellcolor{green!15}{76.4} & \cellcolor{green!15}{65.3} & \cellcolor{green!15}{82.0} & \cellcolor{green!15}{80.9} & \cellcolor{green!15}{64.4} & \cellcolor{green!15}{87.7} & \cellcolor{green!15}{84.1} & \cellcolor{green!15}{98.5} & \cellcolor{green!15}{98.8} & \cellcolor{green!15}{78.5} \\

\bottomrule

\toprule

& & \multicolumn{5}{c}{ETTm1} & \multicolumn{5}{c}{Exchange Rate} & \multicolumn{5}{c}{fMRI} \\

\cmidrule(r){3-7}
\cmidrule(rl){8-12}
\cmidrule(l){13-17}

Generator & Method & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ \\

\midrule

\multirow{2}{*}{SSSD} & DIRE & \textcolor{gray}{85.4} & \textcolor{gray}{87.2} & \textcolor{gray}{93.2} & \textcolor{gray}{87.6} & \textcolor{gray}{79.4} & \textcolor{gray}{71.4} & \textcolor{gray}{77.7} & \textcolor{gray}{97.0} & \textcolor{gray}{97.4} & \textcolor{gray}{65.8} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
& Disjoint-CNN & \textcolor{gray}{99.6} & \textcolor{gray}{99.6} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
\cmidrule{1-17}

\multirow{2}{*}{TSDiff} & DIRE & 80.0 & 81.2 & 85.1 & 87.4 & 0.00 & 53.1 & 50.8 & 57.9 & 50.5 & 0.00 & 66.7 & 50.0 & 90.7 & 94.9 & 0.00 \\
& Disjoint-CNN & 99.0 & 99.0 & 100. & 100. & 98.9 & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. \\
\cmidrule{1-17}

\multirow{2}{*}{Diffusion-TS} & DIRE & 60.5 & 51.0 & 50.3 & 50.8 & 0.00 & 45.5 & 33.2 & 38.5 & 27.9 & 0.00 & 66.7 & 50.0 & 50.0 & 50.0 & 0.00 \\
& Disjoint-CNN & 76.0 & 68.6 & 93.8 & 94.5 & 39.4 & 77.3 & 70.6 & 96.5 & 97.1 & 50.2 & 66.7 & 50.0 & 92.8 & 94.5 & 26.9 \\
\cmidrule{1-17}

\multirow{2}{*}{WaveStitch} & DIRE & 78.3 & 79.3 & 85.2 & 81.0 & 0.00 & 48.3 & 40.2 & 46.5 & 40.4 & 0.00 & 66.8 & 50.3 & 94.5 & 97.1 & 0.00 \\
& Disjoint-CNN & 98.7 & 98.7 & 100. & 100. & 98.8 & 99.6 & 99.6 & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. \\
\cmidrule{1-17}

\multirow{2}{*}{Avg. OOD} & DIRE & 72.9 & 70.5 & 73.5 & 73.1 & 0.00 & 49.0 & 41.4 & 47.6 & 39.6 & 0.00 & 66.7 & 50.1 & 78.4 & 80.7 & 0.00 \\
& Disjoint-CNN & \cellcolor{green!15}{91.2} & \cellcolor{green!15}{88.7} & \cellcolor{green!15}{97.9} & \cellcolor{green!15}{98.1} & \cellcolor{green!15}{79.0} & \cellcolor{green!15}{92.3} & \cellcolor{green!15}{90.0} & \cellcolor{green!15}{98.8} & \cellcolor{green!15}{99.0} & \cellcolor{green!15}{83.4} & \cellcolor{green!15}{88.9} & \cellcolor{green!15}{83.3} & \cellcolor{green!15}{97.6} & \cellcolor{green!15}{98.2} & \cellcolor{green!15}{75.6} \\

\bottomrule

\toprule

& & \multicolumn{5}{c}{Illness} & \multicolumn{5}{c}{Stock} & \multicolumn{5}{c}{Traffic} \\

\cmidrule(r){3-7}
\cmidrule(rl){8-12}
\cmidrule(l){13-17}

Generator & Method & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ \\

\midrule

\multirow{2}{*}{SSSD} & DIRE & \textcolor{gray}{99.5} & \textcolor{gray}{99.5} & \textcolor{gray}{99.4} & \textcolor{gray}{99.7} & \textcolor{gray}{100.} & \textcolor{gray}{98.5} & \textcolor{gray}{98.5} & \textcolor{gray}{98.9} & \textcolor{gray}{99.4} & \textcolor{gray}{0.00} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
& Disjoint-CNN & \textcolor{gray}{99.2} & \textcolor{gray}{99.2} & \textcolor{gray}{99.3} & \textcolor{gray}{99.5} & \textcolor{gray}{85.8} & \textcolor{gray}{99.9} & \textcolor{gray}{99.9} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
\cmidrule{1-17}

\multirow{2}{*}{TSDiff} & DIRE & 66.7 & 50.0 & 49.9 & 49.8 & 0.00 & 69.7 & 56.6 & 55.2 & 59.4 & 0.00 & 66.7 & 50.0 & 50.0 & 50.0 & 0.00 \\
& Disjoint-CNN & 89.8 & 88.7 & 91.5 & 94.2 & 19.5 & 100. & 100. & 100. & 100. & 100. & 66.7 & 50.0 & 100. & 100. & 100. \\
\cmidrule{1-17}

\multirow{2}{*}{Diffusion-TS} & DIRE & 66.7 & 50.0 & 49.9 & 49.8 & 0.00 & 72.9 & 62.8 & 60.6 & 67.5 & 0.00 & 66.9 & 50.4 & 53.2 & 56.1 & 0.00 \\
& Disjoint-CNN & 72.0 & 61.1 & 41.5 & 41.1 & 0.00 & 82.7 & 79.1 & 86.9 & 94.0 & 0.57 & 66.7 & 50.0 & 40.8 & 40.1 & 0.19 \\
\cmidrule{1-17}

\multirow{2}{*}{WaveStitch} & DIRE & 66.7 & 50.0 & 52.4 & 54.7 & 0.00 & 71.5 & 60.1 & 64.1 & 72.0 & 0.00 & 66.7 & 50.0 & 50.0 & 50.0 & 0.00 \\
& Disjoint-CNN & 94.9 & 94.6 & 86.2 & 94.4 & 0.00 & 99.2 & 99.1 & 100. & 100. & 100. & 100. & 100. & 100. & 100. & 100. \\
\cmidrule{1-17}

\multirow{2}{*}{Avg. OOD} & DIRE & 66.7 & 50.0 & 50.8 & 51.4 & 0.00 & 71.4 & 59.8 & 60.0 & 66.3 & 0.00 & 66.7 & 50.1 & 51.1 & 52.0 & 0.00 \\
& Disjoint-CNN & \cellcolor{green!15}{85.6} & \cellcolor{green!15}{81.5} & \cellcolor{green!15}{73.1} & \cellcolor{green!15}{76.6} & \cellcolor{green!15}{6.50} & \cellcolor{green!15}{94.0} & \cellcolor{green!15}{92.8} & \cellcolor{green!15}{95.6} & \cellcolor{green!15}{98.0} & \cellcolor{green!15}{66.9} & \cellcolor{green!15}{77.8} & \cellcolor{green!15}{66.7} & \cellcolor{green!15}{80.3} & \cellcolor{green!15}{80.0} & \cellcolor{green!15}{66.7} \\

\bottomrule

\toprule

& & \multicolumn{5}{c}{Weather} \\

\cmidrule{3-17}

Generator & Method & F1 $\uparrow$ & Acc. $\uparrow$ & AP $\uparrow$ & AUC $\uparrow$ & TPR $\uparrow$ \\

\midrule

\multirow{2}{*}{SSSD} & DIRE & \textcolor{gray}{99.8} & \textcolor{gray}{99.9} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{99.9} \\
& Disjoint-CNN & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} & \textcolor{gray}{100.} \\
\cmidrule{1-17}

\multirow{2}{*}{TSDiff} & DIRE & 66.6 & 49.9 & 49.9 & 49.8 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 97.9 & 98.5 & 55.2 \\
\cmidrule{1-17}

\multirow{2}{*}{Diffusion-TS} & DIRE & 66.6 & 49.9 & 49.9 & 49.9 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 50.7 & 51.6 & 0.78 \\
\cmidrule{1-17}

\multirow{2}{*}{WaveStitch} & DIRE & 66.7 & 50.2 & 50.3 & 50.5 & 0.00 \\
& Disjoint-CNN & 66.7 & 50.0 & 86.0 & 87.2 & 17.0 \\
\cmidrule{1-17}

\multirow{2}{*}{Avg. OOD} & DIRE & 66.6 & 50.0 & 50.0 & 50.1 & 0.00 \\
& Disjoint-CNN & \cellcolor{green!15}{66.7} & \cellcolor{green!15}{50.0} & \cellcolor{green!15}{78.2} & \cellcolor{green!15}{79.1} & \cellcolor{green!15}{24.3} \\

\bottomrule
\end{tabular}
}
\end{table}

==> src/tables/quality_128.tex <==
\begin{table}[ht!]

\centering
\caption{Synthetic time series quality of each generator across ten datasets for \textit{128-length} sequences. All metrics are lower the better.}
\label{tab:quality_128}
% \resizebox{\linewidth}{!}{
\begin{tabular}{llcccc}

\toprule

Dataset & Generator & Context-FID $\downarrow$ & Correlational $\downarrow$ & Discriminative $\downarrow$ & Predictive $\downarrow$ \\

\midrule

\multirow{4}{*}{Electricity} & SSSD & \val{615.3}{44.4}{} & \val{2547}{11}{} & \val{0.500}{0.000}{} & \val{1.175}{0.107}{} \\
& TSDiff & \val{50.76}{1.65}{} & \val{1927}{12}{} & \val{0.500}{0.000}{} & \val{0.835}{0.002}{} \\
& Diffusion-TS & \val{7.571}{0.428}{} & \val{410.5}{10.3}{} & \val{0.500}{0.000}{} & \val{0.815}{0.009}{} \\
& WaveStitch & \val{651.0}{33.7}{} & \val{2553}{11}{} & \val{0.500}{0.000}{} & \val{1.168}{0.121}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Energy} & SSSD & \val{187.8}{40.7}{} & \val{12.78}{0.13}{} & \val{0.500}{0.000}{} & \val{0.927}{0.038}{} \\
& TSDiff & \val{115.4}{29.7}{} & \val{11.81}{0.07}{} & \val{0.500}{0.000}{} & \val{0.924}{0.055}{} \\
& Diffusion-TS & \val{17.36}{3.23}{} & \val{7.318}{0.155}{} & \val{0.500}{0.000}{} & \val{0.901}{0.025}{} \\
& WaveStitch & \val{259.7}{55.1}{} & \val{13.30}{0.12}{} & \val{0.500}{0.000}{} & \val{0.889}{0.016}{} \\

\cmidrule{1-6}

\multirow{4}{*}{ETTh1} & SSSD & \val{124.2}{31.0}{} & \val{0.565}{0.003}{} & \val{0.500}{0.000}{} & \val{1.221}{0.010}{} \\
& TSDiff & \val{22.13}{1.69}{} & \val{0.331}{0.012}{} & \val{0.500}{0.000}{} & \val{1.218}{0.076}{} \\
& Diffusion-TS & \val{35.03}{9.45}{} & \val{0.438}{0.006}{} & \val{0.484}{0.004}{} & \val{1.329}{0.025}{} \\
& WaveStitch & \val{130.4}{40.3}{} & \val{0.554}{0.006}{} & \val{0.500}{0.000}{} & \val{1.238}{0.015}{} \\

\cmidrule{1-6}

\multirow{4}{*}{ETTm1} & SSSD & \val{5169}{1608}{} & \val{0.508}{0.002}{} & \val{0.500}{0.000}{} & \val{1.821}{0.075}{} \\
& TSDiff & \val{15.86}{0.89}{} & \val{0.672}{0.004}{} & \val{0.498}{0.001}{} & \val{1.274}{0.027}{} \\
& Diffusion-TS & \val{25.91}{3.18}{} & \val{0.432}{0.004}{} & \val{0.453}{0.002}{} & \val{1.359}{0.023}{} \\
& WaveStitch & \val{545.1}{51.7}{} & \val{0.520}{0.006}{} & \val{0.500}{0.000}{} & \val{1.235}{0.030}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Exchange Rate} & SSSD & \val{192.5}{59.3}{} & \val{1.504}{0.010}{} & \val{0.500}{0.000}{} & \val{1.270}{0.203}{} \\
& TSDiff & \val{39.78}{6.99}{} & \val{1.252}{0.025}{} & \val{0.500}{0.000}{} & \val{1.163}{0.196}{} \\
& Diffusion-TS & \val{142.1}{63.8}{} & \val{0.928}{0.023}{} & \val{0.500}{0.000}{} & \val{0.968}{0.029}{} \\
& WaveStitch & \val{50.37}{12.12}{} & \val{1.051}{0.018}{} & \val{0.500}{0.000}{} & \val{1.003}{0.058}{} \\

\cmidrule{1-6}

\multirow{4}{*}{fMRI} & SSSD & \val{25.89}{3.57}{} & \val{18.35}{0.04}{} & \val{0.500}{0.000}{} & \val{0.798}{0.001}{} \\
& TSDiff & \val{34.09}{0.44}{} & \val{10.09}{0.01}{} & \val{0.500}{0.000}{} & \val{0.798}{0.000}{} \\
& Diffusion-TS & \val{7.015}{0.097}{} & \val{3.340}{0.026}{} & \val{0.499}{0.001}{} & \val{0.822}{0.003}{} \\
& WaveStitch & \val{33.88}{4.11}{} & \val{23.33}{0.03}{} & \val{0.500}{0.000}{} & \val{0.899}{0.019}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Illness} & SSSD & \val{18.96}{1.38}{} & \val{0.169}{0.009}{} & \val{0.500}{0.000}{} & \val{1.108}{0.006}{} \\
& TSDiff & \val{60.64}{27.87}{} & \val{0.234}{0.026}{} & \val{0.496}{0.005}{} & \val{1.108}{0.006}{} \\
& Diffusion-TS & \val{89.90}{42.87}{} & \val{0.212}{0.016}{} & \val{0.500}{0.000}{} & \val{1.107}{0.003}{} \\
& WaveStitch & \val{19.44}{0.86}{} & \val{0.369}{0.020}{} & \val{0.500}{0.000}{} & \val{1.103}{0.004}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Stock} & SSSD & \val{18.63}{3.34}{} & \val{0.094}{0.012}{} & \val{0.500}{0.000}{} & \val{1.024}{0.015}{} \\
& TSDiff & \val{12.98}{2.17}{} & \val{0.029}{0.014}{} & \val{0.500}{0.000}{} & \val{1.253}{0.104}{} \\
& Diffusion-TS & \val{79.33}{52.47}{} & \val{0.094}{0.010}{} & \val{0.499}{0.001}{} & \val{1.007}{0.008}{} \\
& WaveStitch & \val{22.01}{7.25}{} & \val{0.248}{0.009}{} & \val{0.500}{0.000}{} & \val{1.933}{0.092}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Traffic} & SSSD & \val{419.9}{16.6}{} & \val{20967}{101}{} & \val{0.500}{0.000}{} & \val{1.221}{0.088}{} \\
& TSDiff & \val{60.36}{4.13}{} & \val{10089}{148}{} & \val{0.500}{0.000}{} & \val{1.030}{0.087}{} \\
& Diffusion-TS & \val{159609055}{14208337}{} & \val{8021}{5733}{} & \val{0.500}{0.000}{} & \val{0.757}{0.004}{} \\
& WaveStitch & \val{418.9}{18.3}{} & \val{20968}{101}{} & \val{0.500}{0.000}{} & \val{1.156}{0.061}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Weather} & SSSD & \val{284.7}{53.7}{} & \val{5.173}{0.015}{} & \val{0.500}{0.000}{} & \val{0.289}{0.069}{} \\
& TSDiff & \val{29.27}{2.55}{} & \val{4.726}{0.020}{} & \val{0.500}{0.000}{} & \val{0.365}{0.040}{} \\
& Diffusion-TS & \val{48.98}{6.91}{} & \val{1.644}{0.033}{} & \val{0.481}{0.009}{} & \val{0.050}{0.001}{} \\
& WaveStitch & \val{568.0}{111.7}{} & \val{6.582}{0.010}{} & \val{0.500}{0.000}{} & \val{0.424}{0.034}{} \\

\bottomrule

\end{tabular}
% }
\end{table}

==> src/tables/quality_32.tex <==
\begin{table}[ht!]

\centering
\caption{Synthetic time series quality of each generator across ten datasets for \textit{32-length} sequences. All metrics are lower the better.}
\label{tab:quality_32}
% \resizebox{\linewidth}{!}{
\begin{tabular}{llcccc}

\toprule

Dataset & Generator & Context-FID $\downarrow$ & Correlational $\downarrow$ & Discriminative $\downarrow$ & Predictive $\downarrow$ \\

\midrule

\multirow{4}{*}{Electricity} & SSSD & \val{309.8}{9.7}{} & \val{2520}{6}{} & \val{0.500}{0.000}{} & \val{0.992}{0.040}{} \\
& TSDiff & \val{20.27}{2.03}{} & \val{929.0}{3.5}{} & \val{0.500}{0.000}{} & \val{0.911}{0.010}{} \\
& Diffusion-TS & \val{4.979}{0.356}{} & \val{410.9}{4.2}{} & \val{0.500}{0.000}{} & \val{0.778}{0.006}{} \\
& WaveStitch & \val{311.5}{8.1}{} & \val{2517}{6}{} & \val{0.500}{0.000}{} & \val{1.077}{0.082}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Energy} & SSSD & \val{10.53}{1.37}{} & \val{10.58}{0.15}{} & \val{0.500}{0.000}{} & \val{0.898}{0.024}{} \\
& TSDiff & \val{38.24}{5.01}{} & \val{15.47}{0.13}{} & \val{0.500}{0.000}{} & \val{0.919}{0.042}{} \\
& Diffusion-TS & \val{10.78}{2.07}{} & \val{7.410}{0.156}{} & \val{0.499}{0.001}{} & \val{0.916}{0.026}{} \\
& WaveStitch & \val{8.805}{0.714}{} & \val{10.02}{0.19}{} & \val{0.500}{0.000}{} & \val{0.861}{0.000}{} \\

\cmidrule{1-6}

\multirow{4}{*}{ETTh1} & SSSD & \val{18.36}{1.98}{} & \val{0.381}{0.006}{} & \val{0.490}{0.002}{} & \val{1.361}{0.016}{} \\
& TSDiff & \val{17.89}{0.50}{} & \val{0.627}{0.007}{} & \val{0.499}{0.001}{} & \val{1.255}{0.022}{} \\
& Diffusion-TS & \val{25.08}{6.40}{} & \val{0.430}{0.009}{} & \val{0.450}{0.009}{} & \val{1.367}{0.016}{} \\
& WaveStitch & \val{19.51}{2.53}{} & \val{0.369}{0.009}{} & \val{0.489}{0.002}{} & \val{1.336}{0.030}{} \\

\cmidrule{1-6}

\multirow{4}{*}{ETTm1} & SSSD & \val{16.87}{2.39}{} & \val{0.422}{0.007}{} & \val{0.482}{0.002}{} & \val{1.276}{0.012}{} \\
& TSDiff & \val{19.27}{2.75}{} & \val{0.612}{0.010}{} & \val{0.500}{0.000}{} & \val{1.481}{0.010}{} \\
& Diffusion-TS & \val{19.23}{2.77}{} & \val{0.426}{0.005}{} & \val{0.412}{0.001}{} & \val{1.416}{0.028}{} \\
& WaveStitch & \val{13.64}{2.04}{} & \val{0.448}{0.008}{} & \val{0.475}{0.006}{} & \val{1.220}{0.008}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Exchange Rate} & SSSD & \val{17.01}{4.41}{} & \val{1.165}{0.024}{} & \val{0.500}{0.000}{} & \val{1.280}{0.179}{} \\
& TSDiff & \val{23.13}{5.80}{} & \val{1.095}{0.017}{} & \val{0.500}{0.000}{} & \val{1.442}{0.388}{} \\
& Diffusion-TS & \val{73.10}{45.27}{} & \val{0.948}{0.013}{} & \val{0.500}{0.000}{} & \val{0.952}{0.018}{} \\
& WaveStitch & \val{17.92}{3.94}{} & \val{1.272}{0.010}{} & \val{0.500}{0.000}{} & \val{1.200}{0.213}{} \\

\cmidrule{1-6}

\multirow{4}{*}{fMRI} & SSSD & \val{13.84}{0.23}{} & \val{5.896}{0.025}{} & \val{0.498}{0.002}{} & \val{0.802}{0.001}{} \\
& TSDiff & \val{13.21}{0.20}{} & \val{10.33}{0.05}{} & \val{0.499}{0.000}{} & \val{0.829}{0.006}{} \\
& Diffusion-TS & \val{1.644}{0.040}{} & \val{4.031}{0.064}{} & \val{0.477}{0.005}{} & \val{0.845}{0.003}{} \\
& WaveStitch & \val{14.00}{0.17}{} & \val{5.801}{0.036}{} & \val{0.497}{0.002}{} & \val{0.796}{0.002}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Illness} & SSSD & \val{10.20}{0.52}{} & \val{0.263}{0.055}{} & \val{0.493}{0.006}{} & \val{1.240}{0.005}{} \\
& TSDiff & \val{15.56}{1.20}{} & \val{0.403}{0.080}{} & \val{0.499}{0.003}{} & \val{1.328}{0.039}{} \\
& Diffusion-TS & \val{14.42}{1.52}{} & \val{0.165}{0.038}{} & \val{0.489}{0.013}{} & \val{1.235}{0.006}{} \\
& WaveStitch & \val{10.88}{0.60}{} & \val{0.238}{0.034}{} & \val{0.494}{0.005}{} & \val{1.248}{0.006}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Stock} & SSSD & \val{11.29}{1.39}{} & \val{0.016}{0.012}{} & \val{0.500}{0.000}{} & \val{1.043}{0.064}{} \\
& TSDiff & \val{9.641}{1.587}{} & \val{0.158}{0.020}{} & \val{0.500}{0.001}{} & \val{1.024}{0.019}{} \\
& Diffusion-TS & \val{58.39}{37.76}{} & \val{0.100}{0.007}{} & \val{0.500}{0.001}{} & \val{0.997}{0.001}{} \\
& WaveStitch & \val{10.07}{1.45}{} & \val{0.013}{0.012}{} & \val{0.500}{0.001}{} & \val{0.997}{0.001}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Traffic} & SSSD & \val{287.8}{10.8}{} & \val{20913}{98}{} & \val{0.500}{0.000}{} & \val{1.140}{0.061}{} \\
& TSDiff & \val{29.51}{1.43}{} & \val{13202}{134}{} & \val{0.500}{0.000}{} & \val{0.988}{0.011}{} \\
& Diffusion-TS & \val{41721219}{4298762}{} & \val{12625}{3555}{} & \val{0.500}{0.000}{} & \val{0.757}{0.004}{} \\
& WaveStitch & \val{287.0}{11.1}{} & \val{20912}{98}{} & \val{0.500}{0.000}{} & \val{1.161}{0.015}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Weather} & SSSD & \val{7.916}{0.682}{} & \val{3.238}{0.042}{} & \val{0.497}{0.000}{} & \val{0.112}{0.025}{} \\
& TSDiff & \val{21.43}{3.16}{} & \val{3.017}{0.035}{} & \val{0.500}{0.000}{} & \val{0.351}{0.029}{} \\
& Diffusion-TS & \val{5.772}{0.658}{} & \val{1.623}{0.107}{} & \val{0.428}{0.004}{} & \val{0.052}{0.000}{} \\
& WaveStitch & \val{8.116}{0.725}{} & \val{2.747}{0.045}{} & \val{0.496}{0.001}{} & \val{0.110}{0.024}{} \\

\bottomrule

\end{tabular}
% }
\end{table}

==> src/tables/quality_64.tex <==
\begin{table}[ht!]

\centering
\caption{Synthetic time series quality of each generator across ten datasets for \textit{64-length} sequences. All metrics are lower the better.}
\label{tab:quality_64}
% \resizebox{\linewidth}{!}{
\begin{tabular}{llcccc}

\toprule

Dataset & Generator & Context-FID $\downarrow$ & Correlational $\downarrow$ & Discriminative $\downarrow$ & Predictive $\downarrow$ \\

\midrule

\multirow{4}{*}{Electricity} & SSSD & \val{401.2}{17.1}{} & \val{2518}{13}{} & \val{0.500}{0.000}{} & \val{1.051}{0.030}{} \\
& TSDiff & \val{30.33}{2.27}{} & \val{1448}{16}{} & \val{0.500}{0.000}{} & \val{0.847}{0.007}{} \\
& Diffusion-TS & \val{6.875}{0.653}{} & \val{412.0}{10.8}{} & \val{0.500}{0.000}{} & \val{0.796}{0.006}{} \\
& WaveStitch & \val{402.4}{16.4}{} & \val{2520}{13}{} & \val{0.500}{0.000}{} & \val{1.093}{0.132}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Energy} & SSSD & \val{12.11}{1.79}{} & \val{9.325}{0.089}{} & \val{0.500}{0.000}{} & \val{1.051}{0.049}{} \\
& TSDiff & \val{157.2}{26.1}{} & \val{18.77}{0.06}{} & \val{0.500}{0.000}{} & \val{0.891}{0.007}{} \\
& Diffusion-TS & \val{13.54}{3.19}{} & \val{7.444}{0.172}{} & \val{0.500}{0.000}{} & \val{0.906}{0.030}{} \\
& WaveStitch & \val{14.14}{2.28}{} & \val{11.29}{0.07}{} & \val{0.500}{0.000}{} & \val{0.992}{0.045}{} \\

\cmidrule{1-6}

\multirow{4}{*}{ETTh1} & SSSD & \val{33.78}{2.72}{} & \val{0.461}{0.018}{} & \val{0.498}{0.000}{} & \val{1.349}{0.045}{} \\
& TSDiff & \val{8.846}{0.405}{} & \val{0.623}{0.009}{} & \val{0.495}{0.002}{} & \val{1.173}{0.000}{} \\
& Diffusion-TS & \val{28.56}{4.68}{} & \val{0.440}{0.020}{} & \val{0.473}{0.003}{} & \val{1.306}{0.023}{} \\
& WaveStitch & \val{31.64}{3.76}{} & \val{0.368}{0.005}{} & \val{0.497}{0.001}{} & \val{1.387}{0.046}{} \\

\cmidrule{1-6}

\multirow{4}{*}{ETTm1} & SSSD & \val{16.43}{1.33}{} & \val{0.321}{0.004}{} & \val{0.490}{0.001}{} & \val{1.249}{0.010}{} \\
& TSDiff & \val{36.65}{2.03}{} & \val{0.494}{0.003}{} & \val{0.497}{0.001}{} & \val{1.360}{0.058}{} \\
& Diffusion-TS & \val{21.81}{2.12}{} & \val{0.430}{0.007}{} & \val{0.436}{0.004}{} & \val{1.428}{0.027}{} \\
& WaveStitch & \val{17.61}{1.40}{} & \val{0.331}{0.009}{} & \val{0.491}{0.001}{} & \val{1.200}{0.004}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Exchange Rate} & SSSD & \val{23.45}{4.97}{} & \val{1.196}{0.011}{} & \val{0.500}{0.000}{} & \val{1.172}{0.178}{} \\
& TSDiff & \val{35.30}{6.34}{} & \val{1.408}{0.008}{} & \val{0.500}{0.000}{} & \val{1.374}{0.327}{} \\
& Diffusion-TS & \val{89.08}{38.08}{} & \val{0.952}{0.010}{} & \val{0.500}{0.000}{} & \val{1.005}{0.030}{} \\
& WaveStitch & \val{25.40}{5.95}{} & \val{0.989}{0.048}{} & \val{0.500}{0.000}{} & \val{0.983}{0.036}{} \\

\cmidrule{1-6}

\multirow{4}{*}{fMRI} & SSSD & \val{14.00}{0.61}{} & \val{29.26}{0.20}{} & \val{0.500}{0.000}{} & \val{0.850}{0.006}{} \\
& TSDiff & \val{19.64}{0.32}{} & \val{10.75}{0.03}{} & \val{0.500}{0.001}{} & \val{0.823}{0.004}{} \\
& Diffusion-TS & \val{3.568}{0.070}{} & \val{3.757}{0.039}{} & \val{0.495}{0.003}{} & \val{0.833}{0.003}{} \\
& WaveStitch & \val{15.49}{0.58}{} & \val{24.77}{0.07}{} & \val{0.500}{0.000}{} & \val{0.811}{0.001}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Illness} & SSSD & \val{12.96}{1.79}{} & \val{0.258}{0.027}{} & \val{0.498}{0.003}{} & \val{1.185}{0.003}{} \\
& TSDiff & \val{34.13}{12.75}{} & \val{0.277}{0.014}{} & \val{0.500}{0.000}{} & \val{1.217}{0.007}{} \\
& Diffusion-TS & \val{81.64}{40.54}{} & \val{0.161}{0.031}{} & \val{0.495}{0.006}{} & \val{1.191}{0.004}{} \\
& WaveStitch & \val{19.26}{4.29}{} & \val{0.211}{0.017}{} & \val{0.500}{0.000}{} & \val{1.201}{0.013}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Stock} & SSSD & \val{11.75}{1.13}{} & \val{0.158}{0.011}{} & \val{0.500}{0.000}{} & \val{1.254}{0.096}{} \\
& TSDiff & \val{13.19}{3.16}{} & \val{0.284}{0.017}{} & \val{0.499}{0.001}{} & \val{1.311}{0.143}{} \\
& Diffusion-TS & \val{54.14}{26.88}{} & \val{0.102}{0.017}{} & \val{0.500}{0.000}{} & \val{1.003}{0.008}{} \\
& WaveStitch & \val{13.62}{2.89}{} & \val{0.133}{0.014}{} & \val{0.500}{0.000}{} & \val{1.001}{0.002}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Traffic} & SSSD & \val{349.6}{10.5}{} & \val{20944}{138}{} & \val{0.500}{0.000}{} & \val{1.288}{0.041}{} \\
& TSDiff & \val{44.98}{1.96}{} & \val{15755}{216}{} & \val{0.500}{0.000}{} & \val{0.819}{0.008}{} \\
& Diffusion-TS & \val{52.60}{4.98}{} & \val{4232}{3410}{} & \val{0.500}{0.000}{} & \val{0.761}{0.002}{} \\
& WaveStitch & \val{350.2}{8.5}{} & \val{20944}{138}{} & \val{0.500}{0.000}{} & \val{1.117}{0.079}{} \\

\cmidrule{1-6}

\multirow{4}{*}{Weather} & SSSD & \val{101.6}{19.0}{} & \val{4.160}{0.028}{} & \val{0.500}{0.000}{} & \val{0.206}{0.025}{} \\
& TSDiff & \val{25.36}{1.88}{} & \val{3.013}{0.048}{} & \val{0.500}{0.001}{} & \val{0.340}{0.023}{} \\
& Diffusion-TS & \val{20.26}{3.27}{} & \val{1.651}{0.045}{} & \val{0.455}{0.005}{} & \val{0.052}{0.001}{} \\
& WaveStitch & \val{113.2}{16.5}{} & \val{6.656}{0.033}{} & \val{0.500}{0.000}{} & \val{0.305}{0.055}{} \\

\bottomrule

\end{tabular}
% }
\end{table}
